Ellipsoid Fitting Up to a Constant

In [Sau11,SPW13], Saunderson, Parrilo and Willsky asked the following elegant geometric question: what is the largest $m= m(d)$ such that there is an ellipsoid in $\mathbb{R}^d$ that passes through $v_1, v_2, \ldots, v_m$ with high probability when the $v_i$s are chosen independently from the standard Gaussian distribution $N(0,I_{d})$. The existence of such an ellipsoid is equivalent to the existence of a positive semidefinite matrix $X$ such that $v_i^{\top}X v_i =1$ for every $1 \leq i \leq m$ - a natural example of a random semidefinite program. SPW conjectured that $m= (1-o(1)) d^2/4$ with high probability. Very recently, Potechin, Turner, Venkat and Wein and Kane and Diakonikolas proved that $m \geq d^2/\log^{O(1)}(d)$ via certain explicit constructions. In this work, we give a substantially tighter analysis of their construction to prove that $m \geq d^2/C$ for an absolute constant $C>0$. This resolves one direction of the SPW conjecture up to a constant. Our analysis proceeds via the method of Graphical Matrix Decomposition that has recently been used to analyze correlated random matrices arising in various areas [BHK+19]. Our key new technical tool is a refined method to prove singular value upper bounds on certain correlated random matrices that are tight up to absolute dimension-independent constants. In contrast, all previous methods that analyze such matrices lose logarithmic factors in the dimension.

==> dense-norm.tex <==
% \section{Towards tight graph matrix norm bounds: think local, walk global }
% Let's start with some set-up and an overview description of matrix norm bounds.
% \subsection{Overview of a machinery for tight graph matrix norm bounds}
% Our main idea is the following, for any $q\in \N$,
% \begin{align*}
%     \E[\tr \left((M_\al M_\al^T)^{q} \right)] &= \sum_{P:\text{length-q closed walk}} \E[\val(P)]\\
%     &= \sum_{P:\text{length-q closed walk}} \E\left[\prod_{e\in P} \chi_e \right]\\
%     &=\sum_{P:\text{length-q closed walk}} \prod_{e\in P} \E\left[\chi_e^{\mul_P(e)}\right]
%     \end{align*}
%     where $\mul_P(e)$ counts the multiplicity of edge $e$ in walk $P$, and the last equality follows by independence of edge-characters in our setting.
% Putting ourselves into the shoes of a walker, we observe that each step in the walk makes two types of contributions to the final expected trace,\begin{enumerate}
%     \item A combinatorial factor as we decide how the walk proceeds, \emph{vertex factor};
%     \item An edge-value factor as each edge character (counting multiplicities) contributes to the final walk value, \emph{edge factor}. 
% \end{enumerate}
% More concretely, as each edge-character we consider is going to be mean $0$ (eg. in the basic setting of $H_1$ edge, each edge character is simply an i.i.d. Gaussian),  it suffices for us to consider the walk's that use each edge at least twice. The even-ness of a contributing walk motivates the following edge-assignment scheme in the simplest setting for $H_1$-edge, 
% \begin{mdframed}{Edge-value assignment for $H_1$ edge}
% \begin{enumerate}
%     \item Assign a value $\frac{1}{\sqrt{d}}$ for the first ($F$) and last ($R$) appearances;
%     \item Assign a value of at most $\sqrt{\frac{2q}{d}}$ for each middle ($H$) appearance,
% \end{enumerate}
% \end{mdframed}
% Now we claim that the above edge-value assignment scheme is sound, as it gives us an upper bound on the edge-value factor for each edge. On the one hand, for any edge-character that appears exactly twice, our edge assignment is exact as \[ 
% \E[\chi_e^2] = \frac{1}{d} = (\frac{1}{\sqrt{d}})^2
% \] 
% On the other hand, for those that appear more than twice, i.e., for edge multiplicity $t>2$, we have \[ 
% \E[\chi_e^t] = \frac{(t-1)!!}{\sqrt{d}^t} \leq\frac{t^{t/2}}{\sqrt{d}^t}\leq \left( \frac{\sqrt{t}}{\sqrt{d}}\right) \leq \left( \frac{\sqrt{2q}}{\sqrt{d}}\right)
% \]
% where the last equality follows as each edge appears at most $2q$ times in the walk as we consider a length-$2q$ block walk, and each edge may appear at most once within each block.

% With the set-up for edge-value assignment, we are ready to delve into the vertex-factor component, which would be the bulk of our analysis and our major improvement over prior works. For starters, we first describe an approach that gets the correct leading-order terms that matches the so-called saying of ''square-root per vertex outside the separator''. 
% \paragraph{Getting the leading-order term}
% For starters, we note that for a given closed-walk and a prescribed starting point, we have two natural ways of traversing the walk, as we can either traverse the walk following the given direction, or we can traverse it in the reversed direction. The same idea extends to each block, as we can either traverse it from $U_\al$, or from $V_{\al}$, and thus it suffices to bound the vertex factors by the (geometric) average of both traversals. 
\jnote{move below to paper intro?}
\begin{comment}
On a high-level, we demonstrate how this may be helpful for obtaining the square-root factor for a simple line-shape, in particular, the $\tilde{O}(\sqrt{n})$-norm bound for an $n\times n$ GOE matrix under the normalization that each entry is i.i.d. sample from $\N(0,1)$. Consider a given block with only one edge, suppose we are traversing from $U_\al$ to $V_\al$, let $B(U\rightarrow V)$ be the upper bound for the given block along the $U\rightarrow V$  direction, we case on whether this is the first appearance on the $U\rightarrow V$ direction,\begin{enumerate}
	\item if so, $B(U \rightarrow V)=n$ as we pick up a full vertex factor when using a new edge;
	\item however, if we consider the traversal on the reverse direction, since the edge needs to appear at least twice in the walk, this edge would be ''seen'' by the given block, i.e., this would either be an $R$ or $H$ edge, giving us a value of $\Theta(\poly(q))$.
	\item Taking the average gives us a bound of $\Theta(\sqrt{n\poly (q)})$, and the desired bound follows as we typically take $q=\polylog(n)$.
\end{enumerate}

\paragraph{Shaving the logs whenever unnecessary}
To improve upon the prior bounds, we first observe that the vertex-factor for an $R$ edge is potentially loose where we use a factor of $q$. Following our discussion on the simple example of line-graph, a potential reason for unforced return is ''surprise-visit'', i.e., edges that lead to vertices seen so far in the walk. 
Each surprise visit, on the one hand, potentially poses confusion for incident vertices when using $R$ edges from them, while it also comes up a gap of $\frac{q}{n } = \frac{\polylog n}{ n}$ where we observe that each surprise visit comes with a loss of entropy as it goes to visited vertices, hence incurring a loss in the vertex factors at its creation. This begets our main idea that as long as surprise visit does not create too many confusion for $R$-edges, we can use the $\frac{q}{n }$ to settle unforced-return confusion. A similar idea extends to $H$ edges as well where each edge comes with a factor $q$ blow-up over $F/R$ edge within our assignment scheme, while we further observe that it comes with a loss of vertex factor when combined and this offers a desired gap for charging. 

More generally, the focus of shaving the logs due to $R/H$ edges comes from identifying a gap (eg. surprise visit) for each potential confusion, and show that we can assign potential confusions such that each gap is not charged to ''too-many'' potential confusions or $\log$ factors in full generality .

\paragraph{Some logs are real}
to-add-discussion that not all logs can be shaved, and we can in fact show lower bound for the trace, and therefore, the norm.
\end{comment}
\subsection{Return bound for $A^{-1}$ gadgets}
\begin{definition}[Surprise visit]
We call a step in the walk a surprise visit if it uses a new edge to arrive at a visited vertex (that appears before the current block) in the walk.
\end{definition}


\begin{remark} \label{remark: second-F-not-surprise}
It shall be pointed out that in a block-step walk, if we choose to process edges in order, an edge that leads to a visited vertex is not necessarily a surprise visit as it may be opened up by another edge in the current block. 
\end{remark}

\begin{definition}[Dormant step]
We call an edge pushed out from a square vertex a \emph{dormant} visit if this is an $R$ edge and part of some gadget from $M_D$.
\end{definition}
\begin{remark}
It is crucial to notice that each dormant step is either along an $H_2$ or $H_4$ edge in our setting.
\end{remark}
\begin{definition}[High-mul leg]
    Throughout the walk, we call a step using an edge that already appears at least twice by the current step a high-mul leg.
\end{definition}

% \subsubsection{Return bounds for $A^{-1}$ } 
We split the return bound based on circle and square vertices.
\paragraph{Return from circle vertices} 
\begin{definition}[Potential-unforced-return factor for circle vertex $\pur$]
At time $t$, for each vertex $v$, let $\pur_t(v)$ be defined as the following,\begin{enumerate}
		\item Each return leg closed from $v$ contributes an $1$ to $\pur_t(v)$;
		\item Each unclosed $F$ edge currently incident to $v$ contributes an $1$;
		\item An extra $-1$ as we can maintain a counter for each vertex such that there is always one potential return-leg presumed to be forced.	\end{enumerate}
\end{definition}
\begin{lemma}
For any circle vertex $v$ on the boundary of the walk at time $t\in [q]$ in $A^{-1}$, \[ 
\pur_t(v) \leq 2\cdot s_t(v) + h_t(v) 
\] where we define\begin{enumerate}
    \item $s_t(v)$ is the number of surprise visits arriving at $v$ by time $t$;
    \item $h_t(v)$ is the number of high-mul legs arriving at $v$ by time $t$;
\end{enumerate}
\end{lemma}
\begin{proof}
This argument exploits the property of $A^{-1}$ that each circle vertex only gets encoded into the boundary by one edge, and also only pushes out $1$ edge on the boundary of each block, and we give a proof by induction.  Notice this is immediate when vertex $v$ appears for the first time, as there is only an unclosed $F$ edge incident to $v$ (the leg that explores $v$ and this cancels out with the $-1$ in the $\pur$ factor). 

Suppose currently at time $t$ vertex $v$ is on the boundary, and the hypothesis holds, let time $t'$ be the next time $v$ appears on the boundary. The bound follows as we observe the departure from $v$ (along the $U-V$ path) may introduce an $+1$ to $\pur_t(v)$ (assuming $v$ only splits out one edge when on the boundary), and any subsequent arrival at time $t'-1$ either closes an $F$ edge, in which case we have $\pur_t(v) = \pur_{t'}(v)$; otherwise it opens up a new $F$ edge to $v$ (which is a surprise visit) or follow a high-mul leg, and we have an increment of at most $2$ and $1$ respectively in the change of unclosed incident $F$ edges.
\end{proof}

\paragraph{Return bound for square vertices}

\begin{definition}[Potential-unforced-return factor for square vertex $\pur$]
At time $t$, for each vertex $v$, let $\pur_t(v)$ be defined as the following,\begin{enumerate}
		\item Each return leg closed from $v$ contributes an $1$ to $\pur_t(v)$;
		\item Each unclosed $F$ edge currently incident to $v$ contributes an $1$;
		\item An extra $-2$ as we can maintain a counter for each vertex such that there are always two $H_1$ edges (or a pair of $H_2$ edge viewed as two edges) presumed to be forced as each square vertex pushes out two edge-copies a time.\end{enumerate}
\end{definition}
\begin{remark}
Notice the difference between $\pur$ for circle and square factors is only the final subtraction.
\end{remark}
% \begin{definition}[Unsynced pushout and pullback ]
% For each square vertex, and each gadget in which it pushes out (respectively, pulls back) $2$ distinct edges to circle vertices,
% we call it an unsynced pushout (pullback) if two edges receive distinct $F/R/H$ labels.
% \end{definition}
\begin{lemma}
For any square vertex $v$ on the boundary of the walk at time $t\in [q]$ in $M_\al$ and $M_\beta$, \[ 
\pur_t(v) \leq 4\cdot s_t(v) + 4\cdot h_t(v) 
\] where we define\begin{enumerate}
    \item $s_t(v)$ is the number of surprise visits arriving at $v$ by time $t$;
    \item $h_t(v)$ is the number of high-mul legs arriving at $v$ by time $t$;
    %  \item $unsynced_t(v)$ is the number of unsyneced-pushouts from $v$ by time $t$.
\end{enumerate}
\end{lemma}
\begin{proof}
The proof structure is identical to the previous proof for circle vertices, and note that this holds trivially in the base case when $v$ first appears. Suppose this holds for $v$ at time $t$, and let time $t'$ be the subsequent appearance of $v$. Note that the last departure from $v$ opens up at most $2$ $F$ edges, and consider how we arrive back at $v$ at time $t'-1$. 
\begin{itemize}
    \item Suppose we use both $R$ edges in the arrival, this offsets the gain of the at most $2$ new $F$ edges that may be opened up from time $t$ and the hypothesis holds; 
    \item Otherwise, there is at least an $F$ or $H$ edge, and we pick up a gain of at most $4$ new $F$ edges compared to time $t$, thus it suffices to (loosely) assign a gain of $4$ per surprise visit (if $F$ edge) or $H$-visit.
\end{itemize}

\end{proof}
\begin{remark}
To incorporate potential confusion due to dormant step, notice we may a special label that is a constant per step to identify we are using a dormant step, and moreover, for each vertex in our gadget, it has at most $3$ dormant steps each time it appears (unless it comes with extra surprise visit or $H$-visit), and thus the confusion among dormant steps can be further handled at a cost in $O(1)$. 
\end{remark}

\subsection{Generalized Return Bound for $\calI(R)$}
We extend our definitions for surprise visit to intersection terms, which is the starting point for our charging strategy.
\begin{definition}[Generalized surprise visit]
For each block step, following the order given by canonical edge-traversal, we call each new edge that leads to a ''seen'' vertex a \emph{generalized surprise visit}. 
\end{definition}
\begin{remark}
This shall be contrasted with our previous definition of surprise visit, and the modification is made to capture intersections. That said, under this definition, each edge leading to any seen vertex is considered a surprise visit (as long as it is not explored by the current gadget) even though the vertex may be ''new'' for the current block-step as it is discovered by some gadget of current block processed earlier in the canonical ordering for traversal.
\end{remark}

\begin{remark}
This allows a vertex to be reached using both non-surprise visit and surprise visit within the same block.
\end{remark}

\begin{lemma}
For any circle vertex $v$ in $\calI(R)$, let $t$ be a time-mark in the canonical traversal order, we have \[
\pur_t(v)\leq 2\cdot gs_t(v)  +h_t(v)
\]
where $gs_t(v)$ is the counter for generalized surprise visits arriving at $v$.
\end{lemma}

To unify our $\pur$ analysis, we introduce the following,
\begin{definition}[Edge-copy]
We call each $H_1$ edge an edge-copy; moreover, we view each $H_2$ edge $H_2(u,v)$as two separate edge-copies of the same underlying edge $(u,v)$.
\end{definition}

\begin{lemma}[Generalized return bound for square vertices]
For each square vertex $u$, for any time $t$ in the canonical order of traversal, we define $\pur_t(u)$ as the following, \begin{enumerate}
    \item each $R$ edge-copy closed from $u$ by time $t$ contributes an $1$;
    \item each unclosed edge-copy that is also not opened-up as a dormant step from $u$ contributes an $1$;
    \item an extra $-2$ since a square vertex pushes out two edge-copies at at time, and there are two presumed to be fixed.
\end{enumerate} 
When $v$ is on the boundary at time $t$, \[ 
\pur_t(u) \leq 4s_t(u) + 4h_t(u)
\]
for \begin{enumerate}
    \item $s_t(u)$ the number of edge-copies of generalized surprise visits arriving at $u$;
    \item $h_t(u)$ the number of edge-copies of $H$-mul edges arriving at $u$.
\end{enumerate}
\end{lemma}
\begin{proof}
The proof structure is identical to the previous proof for circle vertices, and note that this holds trivially in the base case when $v$ first appears. Suppose this holds for $v$ at time $t$, and let time $t'$ be the subsequent appearance of $v$. Note that the last departure from $v$ opens up at most $2$ $F$ edges, and consider how we arrive back at $v$ at time $t'-1$. 
\begin{itemize}
    \item Suppose we use both $R$ edges in the arrival, this offsets the gain of the at most $2$ new $F$ edges that may be opened up from time $t$ and the hypothesis holds; 
    \item Otherwise, there is at least an $F$ or $H$ edge, and we pick up a gain of at most $4$ new $F$ edges compared to time $t$, thus it suffices to (loosely) assign a gain of $4$ per generalized-surprise visit (if $F$ edge) or $H$-visit.
\end{itemize}
 \end{proof}

% For each block, consider the below process that follows the canonical order of traversal, \begin{enumerate}
%     \item First, connect an auxiliary $U-V$ edge between the two circle vertices, and this is the only edge whose orientation depends on our traversal direction for each block, and moreover, identify both vertices in $U\cup V$ following the auxiliary edge;
%     \item For the edges between $U \cup V$ and the first square vertex in-between, orient both edges to point to the square vertex in the middle;
%     \item For any edges part of the dangling path, orient the edges to point downwards to the subsequent gadget;
%     \item For each traversal direction, label each edge $F/R/H$ including the auxiliary $U-V$ edge; additionally, for each vertex, identify it has a \emph{left constraint edge} if it appears in some block to the left of the current block; similarly, identify a \emph{right constraint edge}  if it appears in some block to the right of the current block;
%     \item Once the \emph{left/right constraint edge} for each vertex is identified (which is equivalent to asking whether each vertex is appearing for the first/middle/last time) while we use left/right constraint edge to get rid of the dependence on traversal direction. 
% \end{enumerate}

% \paragraph{First encounter vertex-factor redistribution}
% Naively, each vertex when it first appears, requires a label of its weight. In particular, any $F$ edge from $u\rightarrow v$ naively requires a label in $\wt(v)$. However, we consider the following scheme that redistributes the vertex factor to the edges noticing the property that $(u,v)$ needs to appear at least twice, regardless of the direction: for any $F$ step $u\rightarrow v$, \begin{enumerate}
%     \item Assign a factor $\sqrt{\wt(v)}$ when $(u,v)$ edge appears as an $F$ step;
%     \item Assign a factor of $\sqrt{\wt(v)}$ when $(u,v)$ edge appears as an $R$ step \emph{regadless of the direction}.
% \end{enumerate}
% Generalizing this to our gadget, we have the following scheme,\begin{enumerate}
%     \item For each pair of edges that discover a ''new'' square vertex: assign each of their $F$ and $R$ copies a weight of $m^{1/4}$ (notice there are $4$ such edge-copies in total);
%      \item For edge that discover a ''new'' circle vertex: assign each of their $F$ and $R$ copies a weight of $\sqrt{d}$;
% \end{enumerate}
% Observe that this is a faithful distribution as each square vertex, when discovered by a pair of edges, require a weight of $m$, and we pick up $4$ factors of $m^{1/4}$ through the $F/R$ appearance of both edge-multiplicity. This holds also for a circle vertex except its weight is distributed to the $F/R$ appearance of the single copy that discovers it.

% Now it suffices for us to consider traversal in arbitrary direction for each block instead of taking average among two traversals. Combining with our gadgets and canonical order of traversal, we can assign vertex factor for each vertex when it first appears being processed as the following, \begin{enumerate}
%     \item $F$ edge: since the direction is fixed, the vertex factor assignment is immediate (i.e. $m^{1/4}$ or $\sqrt{d}$ depending on which new vertex it leads to;
%     \item $R$ edge: modulo the factor needed to specify the choice of $R$ edge captured by $\pur$, we have a back-pay vertex factor depending on which vertex the edge $(u,v)$ leads to when it first appears.  
% \end{enumerate}

% For auxiliary edge, each such edge is not guaranteed to appear twice, and we consider an alternative vertex-factor assignment scheme for vertex-copy in $U\cup V$,\begin{enumerate}
%     \item Assign a factor $\sqrt{d}$ in the block in which it make the first appearance;
%     \item Assign a factor $\sqrt{d}$ in the block in which it makes the last appearance;
% \end{enumerate}
% Since each vertex in $U \cup V$ appears in at least two blocks, this is also a faithful distribution.

% We now keep track of the factors as we follow the canonical order of traversal,
% % \paragraph{$U-V$ auxiliary path} We first remark that this is an auxiliary edge that does not come with edge-value. We follow the previous order of taking average among two possible traversal directions here,
% % \begin{itemize}
% %     \item $F$ step: the edge leads to a new circle vertex, and hence a factor of $d$;
% %     \item $R$ step: modulo the $\pur$ cost for the auxiliary edge, this is a factor of $1$;
% %     \item $S,H$: this incurs a factor of $q^{O(1)}$ via the $\pur$ factor;
% % \end{itemize}
% %  Combining the above gives us a factor of $(1+o_d(1))\cdot  2\sqrt{d}$.
 
%  \paragraph{Half-gadget: from $U$ to $U\cup V$ and dangling start} We remind the reader that following our traversal order, both edges point to the square vertex in the middle, and starting from $U_\al$, the vertex in $V_\al$ is reached first using the auxiliary edge. We employ our vertex factor redistribution scheme here, \begin{enumerate}
%      \item All $F$: at most one of the circle vertices is making their first appearance as well as the middle square vetex, and we pick up edge-value from $2$ $H_1$ edges. Moreover, no vertex can be making their last appearance, hence no back-pay factor is needed nor $\pur$ needed when there is no surprise visit, giving us a bound of \[ 
%      (1+o_d(1)) \cdot \frac{\sqrt{md}}{d}
%      \] 
%      \item All $R$: we need to case on the direction of how the corresponding $F$ copies are opened up for the current $R$ edges in inspection:\begin{itemize}
%          \item if both led to the square vertex in the $F$ copy, we get a back-pay factor of $\sqrt{m}$ from the two edges combined; moreover, at most one of the vertex in $U\cup V$ is making the last appearance which assigns an additional backpay of $\sqrt{d}$, hence we get a factor of $\sqrt{md}$;
%          \item If both led to the circle vertex in the $F$ copy, each edge carry a vertex factor of at most  $\sqrt{d}$, however, observe that there is no boundary backpay needed, we get a bound of $\sqrt{d^2}$;
%          \item If one led to a circle wile another led to a square, 
%      \end{itemize}
     
%      \jnote{issue...fixing..}
%      if all $F$first, the circle vertex reached using auxiliary edge 
     
%      both circle vertices are neither making their first nor last appearance on the boundary, hence no factor needed for them; the square vertex in the middle is either making the first appearance (which would assign it a factor of $\sqrt{m}$) or a surprise visit, hence a factor of \[ 
%      (1+o_d(1)) \cdot \frac{\sqrt{m}}{d} 
%      \]
%      \item $R>--<F$ or $F>--<R$: one of the $F$ edges is a surprise visit, and at most one of the circle vertex is potentially making its last appearance while no vertex (including the square vertex) is making its first appearance, and this gives us a factor of \[ 
%      (1+o_d(1)) \cdot \frac{q^{O(1)}\sqrt{d} }{d} = \tilde{O}(\frac{1}{\sqrt{d}})
%      \]
%      \item The case involving $S,H$ are identical to the above and can be bounded by $\tilde{O}(\frac{1}{\sqrt{d}})$.
%  \end{enumerate}
%  \paragraph{$A^{-1}$-gadget} 
%  We verify by cases, and for each case, we list out the (almost) dominant labelings while any other labeling involving $H$ or surprise visit can be verified to be $o_d(1)$ of the corresponding dominant value. \begin{enumerate}
%      \item $M_\al$ Gadget: we list out the dominant labelingsm that is all $F/R$, or $RR/ FF$ that is constant gap from the dominant term, yielding us a bound of $
%      (1+o_d(1))\cdot \frac{1}{d^2} (2\sqrt{md^2} + \sqrt{m^2})$.
%      \begin{itemize}
%          \item All $F$ (all $R$): no vertex involved is making last (or first) appearance, while at most $2$ circle vertices and one square vertex are making their first (or last) appearance, hence receive a redistributed factor of $\sqrt{md^2}$;
%          \item $RR/FF$: the top and bottom square vertex may be making its last and first appearance respectively, while both of the circle vertices in the middle layer are making their middle appearance, hence no back-pay is needed for them and we pick up  a factor of $(1+o_d(1))\cdot \sqrt{m^2}$ for the two square vertices;
%      \end{itemize}
%      \item $M_\beta$ Gadget: we pick up a factor of $(1+o_d(1)) \frac{2}{d^2} ( 2\sqrt{md} + \sqrt{m^2})$ (identical to the calculation in the toy-example section).
%      \item $M_D$ (Dormant gadgets)
%  \end{enumerate}






\jnote{below is old draft commented out}


\begin{comment}


As a corollary, we obtain the following bound for the block-value of any shape $\al$ that may arise in $\tau(I)$, \begin{align*}
    B(\al) \leq &\sum_{S:\text{separator for }\al } 
\prod_{i\in V(\al)\setminus S}\sqrt{\wt(i)}^{1+1_{iso}(v)} \prod_{e\in E(S)} q^{O(1)} \cdot q^{O(1)\cdot \text{generalized-surprise}(\al) }   \\&\cdot  \prod_{e \in E(\al)\setminus E(S)}\edgeval(F,R) \cdot \prod_{e\in E(S)} \edgeval(H) 
\cdot  \prod_{\substack{i\in S\\ \text{square}}  } q^{O(1)} \cdot (2|V(\al)|q)^{2|\float(\al)|} \numberthis
\end{align*}
where $
\text{generalized-surprise}(\al) $
is the number of generalized-surprise visits if we traverse $\al$ following the canonical-ordering, and notice this number does not depend on the particular choice of separator for $\al$ block.

\subsection{Return is forced for dangling $R$ path}
\paragraph{Forced return bound for circle vertices}
Our starting point here is that when we consider non-intersection term in $\tau(R)$, each circle vertex splits out only one edge when on the walk boundary (which is not necessarily the block boundary $U\cup V$). That said, the return-bound from the previous section almost follows straightforwardly once we address the extra edges that may be pushed out from circle vertex due to intersection. We will then generalize this starting point to capture terms that may arise intersection terms in $\calI(R)$ as well.

% \begin{definition}[Excess pushout leg]
% For each vertex $v$ on the boundary at time $t$, suppose it pushes out $t>1$ edges at the same time, we call all but its first edge an excess pushout leg.
% \end{definition}

% \begin{lemma}
% For any circle vertex $v$ on the boundary of the walk at time $t\in [q]$ in $R$, \[ 
% \pur_t(v) \leq 2\cdot s_t(v) + h_t(v)  + excess_t(v)
% \] where we define\begin{enumerate}
%     \item $s_t(v)$ is the number of surprise visits arriving at $v$ by time $t$;
%     \item $h_t(v)$ is the number of high-mul legs arriving at $v$ by time $t$;
%     % \item $excess_t(v) $ is the number of excess edge pushed-out from $v$ by time $t$ and each edge pushed out from $v$ is an excess if it is not the first edge pushed out from $v$ at this time-mark (i.e., only non-zero when $v$ pushes out multiple edges at a single time-mark on the boundary). 
% \end{enumerate}
% \end{lemma}

\paragraph{Forced return bound for square vertices}
\begin{definition}[Redefined $\pur$ function for square vertices in $R$]
For a square vertex $v$ in $R$, we define its potential unforced return function $\pur(v)$ as the number of $R$ edges closed from $v$ unless the edge is closed when $v$ is making its final appearance, or whose corresponding $F$ edge is opened up from $v$ as a dormant step.
\end{definition}


% \begin{definition}[Redefined $\pur$ function for square vertices in $R$]
% For a square vertex $v$ in $R$, we define its potential unforced return function $\pur(v)$ as the  number of return leg closed from $v$ contributes an $1$ unless it is closed when $v$ is making its final appearance.
% \end{definition}
\begin{remark}
We observe that each unclosed $F$ edge incident to $v$ can be identified as an edge-set for free once we know $v$ is making its final appearance, as they all need to appear in the current block (otherwise we have edges appearing odd number of times which makes the trace vanish).
\end{remark}

\begin{lemma}
For any square vertex $v$ on the boundary of the walk at time $t\in [q]$ in $R$,
\[ 
\pur(v) \leq \left(2 + dormant(v)\right)  \cdot \text{middle-appear}(v) 
\]
where we define \[ 
\text{middle-appear}(v)  = \text{\# of appearances throughout the walk}(v) - 2
\]
and \[
\text{dormant}(v) =\text{\# of $R$ $M_D$ gadget edges pushed out from $v$} 
\]
\end{lemma}
 \begin{proof}
 First, notice a square-vertex may only incur unforced return when it is making its middle appearance, and each time it does so, it pushes out at most $2+ \text{dormant}(v)$ edges, hence our bound follows.
 \end{proof}
 \begin{remark}
 Consider the last appearance of square vertex $v$, the set of edges used is fixed, however, a priori, we need to assign an ordering for the set of edges in the trace moment method, and this is cost of \[ 
3! \max \left(1, (4(dormant_R(u)-1))^{4\cdot (dormant_R(u)-1)}\right)
 \]
 where $dormant_R(u)$ is the number dormant steps called from $u$ when it last appears since 
 \begin{enumerate}
     \item when $dormant_R(u) \leq 1$, a we have at most $3$ edges and hence a cost of $3!$ is sufficient;
     \item for  $dormant_R(u) > 1$, we can assign a label in $dormant_R(u)+2 \leq 4(dormant_R(U)-1)$ for each edge, and we have at most $4(dormant_R(U)-1)$ edges..
 \end{enumerate}
 and notice we get a gap from charging whenever $dormant_R(u) > 1$.
 \end{remark}
 \end{comment}
% \subsubsection{Forced return bound for square vertices}
% The above argument does not apply well directly for square vertices, as it requires processing edges in order and treating any edge that leads to $v$ (except the first discovery leg) a surprise visit, which we can then settle if each surprise visit comes with a gap. However, as pointed out in \cref{remark: second-F-not-surprise}, this is not true in some cases for a square vertex that appear in the $A^{-1}$ gadget (as it can in fact be considered as $2$-in-$2$-out), for example, $M_\al$. 

% To address this issue, we appeal to the observation that each square vertex in our graph matrices can only appear ''twice'' at the boundary, and any further appearance comes with a gap in block-value. In other words, a square vertex can never be inside the separator in the dominant term, and this opens up a gap for recording auxiliary data to ensure the return is ''forced''. While we believe a unified analysis for general graph matrices is within reach, we defer this to future work and give an analysis specialized the matrices that arise in our setting, mainly to avoid unnecessary complications arising from distinct vertex-types and weights.

% For starters, we observe the following property that is satisfied by all shapes that arise in $A^{-1}$ gadget, 
% \begin{observation}[Gadget property]
% For each $A^{-1}$ gadget, each square vertex $s$ may push-out $2$ distinct edges to circle vertices, both of which are connected to another square vertex $t$ (while possibly $s=t$).
% \end{observation}

% Since each time a square vertex pushes out pair of edges, it suffices for us to assume that we can designate $2$ incident unclosed edges to be ''fixed'' as opposed to just one as in the analysis for circle vertices. This prompts us to modify the $\pur$ function for square vertices as the following, 
% \begin{definition}[Potential-unforced-return factor for square vertices $\pur$ ]
% At time $t$, for each square vertex $v$, let $\pur_t(v)$ be defined as the following,\begin{enumerate}
% 		\item Each return leg closed from $v$ contributes an $1$ to $\pur_t(v)$;
% 		\item Each unclosed $F$ edge currently incident to $v$ contributes an $1$;
% 		\item An extra $-2$ as we can maintain a counter for each square vertex such that there is always two potential return-legs presumed to be forced.	\end{enumerate}
% \end{definition}

% \begin{definition}[Unsynced pushout and pullback ]
% For each square vertex, and each gadget in which it pushes out (respectively, pulls back) $2$ distinct edges to circle vertices,
% we call it an unsynced pushout (pullback) if two edges receive distinct $F/R/H$ labels.
% \end{definition}

% For ease of our analysis, we further case on the shapes that appear in $A^{-1}$ and $R$.
% \paragraph{Forced return bound in $A^{-1}$ }
% For the square vertices that arise here, we focus on $M_\al$ and $M_\beta$, and in particular $M_\al$ as this is where our norm bound needs to be tight up-to constant factors.


%\begin{definition}[Redundant-appearances]
% 	For each square vertex that splits out at least two edges in the traversal, we call it a miss-aligned departure if it splits out both $F$ and $R/H$ edges.
% \end{definition}
% \begin{lemma}
% For any circle vertex $v$ on the boundary of the walk, it is incident to at most $
%  2+ 2\cdot s(v) $ unclosed $F$ edges; for any square vertex on the boundary of the walk, it is incident to at most $1 + s(v)$ unclosed $F$ edges where we denote $s(v)$ to be the number of surprise visits arriving at $v$.
% \end{lemma}
% \begin{proof}
% We prove this by induction. Let $s_t(v)$ be the number of surprise visits arriving at $v$ by time $t$, and $h_t(v)$ the number of $H$ visits arriving at $v$. We first consider when $v$ is a square vertex, and observe that when vertex $v$ first appears, the return is fixed as it has only $1$ unclosed $F$ edge; moreover, any subsequent departure may open up an $F$ edge, while the subsequent, unless it closes a previously unclosed $F$ edge, is a surprise visit or an $H$ arrival, hence whenever $v$ is on the boundary, we have \[ 
% pur_t(v) \leq s_t(v) + h_t(v)
% \]
% where $pur_t(v)$ measures the number of potential unforced returns from $v$ by time $t$.
% Analogously for a circle vertex, notice the base case is slightly different as there may be now two edges incident to a circle vertex at each block, and similarly, each departure may open up at most $2$ new $F$ edges. That said, any subsequent arrival at $v$ 
% \end{proof}


% \subsection{Structure lemmas}
% In the following section, we relate the contribution of each block to the separator, and show that the contribution is controlled by the vertex separator. Towards this end, we first observe that for each walk, it can be encoded in two ways, either via a traversal from $U_\al$ to $V_\al$, or via a traversal from $V_\al$ to $U_\al$. 
% \begin{claim}
% For an edge-labeling $\calL$ (presumed to be from $U_\al$ to $V_\al$), its block value is bounded by \[ 
% B(\calL) \leq \sqrt{B(\calL_{U\rightarrow V}) \cdot  B(\calL^T_{V\rightarrow U}) }
% \]
% \end{claim}


% For our first ingredient, we bound the block-value of a given edge-labeling (with fixed traversal direction),
% \begin{claim}
% Let $\calL_{U\rightarrow V}$ be an edge-labeling from $U_\al$ to $V_\al$, its block value is bounded by \[ 
% B(\calL_{U\rightarrow V}) = \vtxcost\cdot \edgeval(\calL)  \leq \prod_{i:\text{new vertex}} \wt(i) \cdot (2q)^{\text{\# vertices arrived by surprise visit}} \cdot q^{ \text{\# of H edges}}
% \]
% \end{claim}


% Fix the traversal direction from $U_\al$ to $V_\al$ while the reciprocal holds in an analogous way once we consider the traversal from $V_\al $ to $U_\al$, \begin{lemma}[No unnecessary turns]
% For any locally optimal labeling, there is unnecessary turn on any path from $U_\al$ to $V_\al$. In other words, any path from $U_\al$ to $V_\al$ is of the form $R\rightarrow H \rightarrow F$ where we allow each edge label-set to be empty.
% \end{lemma}
% \begin{proof}
% Let $\calL$ be an edge-labeling from $U_\al $ to $V_\al$, and let $\calL^T$ be its reciprocal from $V_\al $ to $U_\al$, we will show that its value can be locally improved if it contains an unnecessary turn. For the $M_\al$ we have, it suffices for us to rule out paths of the from $F\rightarrow R$ (as well as $F\rightarrow H$) from $U_\al$ to $V_\al$ (or from $V_\al$ to $U_\al$ if we consider$\calL^T$).

% Suppose there is an $F\rightarrow R$ (or $F\rightarrow H$) path from $U_\al \rightarrow V_\al$, let $S$ be the set of vertices reachable from $U_\al$ via some $F$ path while incident to some $R$ or $H$ edge, and let $S_L$ be the set of vertices in $S$ that are reachable from $U_\al$ without passing through any other vertex in $S$. Let $\calL'$ be the edge-labeling obtained by flipping any $F$ path in $\calL$ into an $R$ path, and it now suffices to show that we have made improvement in the local block value (after averaging over both traversal directions), i.e. ,\[ 
% B(\calL') > B(\calL) 
% \]
% To start with, we first observe that the transpose map $\calL^T$ is well-defined from $\calL$  as \begin{enumerate}
%     \item Any $F$ edge becomes an $R$ edge, and vice versa;
%     \item Any $H$ edge stays remains an $H$ edge.
% \end{enumerate}
% That said, the edge factor stays invariant when we consider the edge-labeling and its transpose; moreover, since we only flip $F$ edges into $R$ edges when we shift from $\calL$ to $\calL'$, the edge factors remain invariant again, i.e., \[ 
% \edgeval(\calL_{U\rightarrow V }) = \edgeval(L_{V\rightarrow U}^T) = \edgeval(\calL_{U\rightarrow V }') = \edgeval(\calL_{V\rightarrow U}'^T)
% \]
% It suffices for us to consider the change in vertex factors. $S_L$ may contain multiple vertices while we can pick an ordering of processing vertices in $S_L$ and apply the following argument inductively. For simplicity, we further assume that $S_L \subseteq V(\al)\setminus U_\al\cup V_\al$ as this is a set of vertices passed through by some $F\rightarrow R/H$ path from $U_\al$ to $V_\al$, and we assume that there are no internal edges with both endpoints in $U_\al$ or in $V_\al$. Let $v$ be such a vertex in $S_L$, a let $F(U_\al, v)$ be the set of vertices any $F$ path from $U_\al$ to $v$ including those in $U_\al$, and we observe the following,
% \begin{enumerate}
%     \item Any vertex in $V(\al)\setminus F(U_\al, v)$ receive the same vertex factor in $\calL$ and $\calL'$ (in particular, they receive the same vertex factor in either traversal direction under $\calL$ and $\calL'$);
%     \item Any vertex in $F(U_\al, v)\setminus (U_\al\cup \{v\})$ receives a full factor of $n$ under $\calL_{U\rightarrow v}$ as they are destinations of $F$ edges, and a factor of $1$ under $\calL_{V\rightarrow U}$ as they are arrived via $R$ edges;
%     \item Any vertex in $F(U_\al, v)\setminus (U_\al\cup \{v\})$ receives a factor of $1$ under $\calL'_{U\rightarrow v}$ as they are destinations of $R$ edge, and a factor of $[n]$ under $\calL'_{V\rightarrow U}$ as they are arrived via $F$ edges;
%     \item Any vertex in $F(U_\al,v)\cap U_\al$ in $\calL$ is fixed when traversing from $U$ to $V$ as they are the boundary encoded from the last block, and receive a factor of $1$ in $\calL^T$ when traversing from $V$ to $U$ as they are arrived via $R$ edges;
%     \item Any vertex in $F(U_\al,v)\cap U_\al$ in $\calL'$ is fixed when traversing from $U$ to $V$ as they are the boundary encoded from the last block, and receive a factor of $[n]$ when traversing from $V$ to $U$ as they are arrived via $F$ edges;
%     \item Vertex $v$ receives a factor of $q$ under $\calL_{U\rightarrow V}$ as it is a vertex seen in some previous block while now arrived using some $F$ edge, and it receives a factor at most $q$ under the traversal from $V$ to $U$ as it is incident to some $R$ edge in $L^T$;
%     \item Vertex $v$ receives a factor of $1$ under $\calL'_{U\rightarrow V}$ as it is arrived using an $R$ edge, and any such vertex $v$ receives a factor $[n]$ under the traversal from $V$ to $U$;
% \end{enumerate}
% Combining the above, we have \[ 
% \frac{\vtxcost(\calL')}{\vtxcost(\calL)}= \Delta(v) \cdot \Delta\left(F(U_\al, v)\cap U_\al\right) \geq  \frac{1}{q}\cdot \prod_{i\in | F(U_\al, v)\cap U_\al|} \sqrt{\wt(i)} \gg 1
% \]
% where we observe that $|F(U_\al, v)\cap U_\al|\geq 1$ by construction as $v$ is passed through by some $U_\al\rightarrow V_\al$ path, and our assumption that $q \leq O(n^{\delta})$.
% \end{proof}
% \begin{lemma}[$H$ edge can be locally improved if the shape has bounded degree] For a shape $\al$ that has bounded degree, i.e., any vertex in $V(\al)$ has $O(1)$ neighbors, for any locally optimal edge-labeling, any path from $U_\al$ to $V_\al$ is of the structure $R\rightarrow F$; in particular, it does not contain any $H$ edge.
% \end{lemma}
% \begin{proof}
% It suffices for us to assume $\calL$ is an edge labeling such that any path from $U_\al$ to $V_\al$ is of the structure $R\rightarrow H\rightarrow F$, and suppose there is a path with $H$ edge from $U_\al$ to $V_\al$, and let $v\rightarrow u$ be the first $H$ edge on this path reachable from $U_\al$. Let $\calL'$ be an alternate edge-labeling obtained by flipping the edge $v\rightarrow u$ from $H$ to $R$, and we claim that $B(\calL')> B(\calL)$. As we observe the following,
% \begin{enumerate}
%     \item Any vertex $w\in V(\al)\setminus \{u,v\}$ receives the same vertex factor under $\calL$ and $\calL'$ (in particular, it receives the same vertex factor in either traversal direction);
%     \item Any edge in $E(\al)$ not incident to $v$ receives the same edge factor under $\calL$ and $\calL'^T$;
%     \item Vertex $v$ receives $O(1)$ vertex factor in $\calL$ from $U\rightarrow V$ as it is reachable from an $R$ edge, and a factor of at most $q$ in $\calL^T$ from $V\rightarrow U$ as it is reachable from an $H$ edge;
%     \item  Vertex $v$ receives $O(1)$ vertex factor in $\calL'$ from $U\rightarrow V$ as it is reachable from an $R$ edge, and a factor of $O(1)$ in $\calL'^T$ from $V\rightarrow U$ as it is reachable from an $R$ edge (since the $u\rightarrow v$ edge is now an $F$ edge, and any path from $v$ to $U_\al$ is $F$);
%     \item Vertex $u$ receives a vertex factor of at most $q$ in $\calL$ from $U\rightarrow V$ as it is reachable from an $H$ edge, and a factor of $f_{\calL^T}(u)$ in $\calL^T$ from $V\rightarrow U$;
%     \item Vertex $u$ receives a vertex of $1$ in $\calL'$ from $U\rightarrow V$ as it is reachable an $R$ edge, while a vertex factor of at least  $f_{\calL^T}(u)$ in $\calL^T$ from $V\rightarrow U$ as the only change of $\calL'^T$ from $\calL^T$ is an incident edge to $u$ flips from $H$ to $F$, which does not decrease the vertex factor for $u$;
%     \item The edge value of any edge (eg. the edge $(u,v)$) incident to $v$ was $q$ in both $\calL$ and $\calL^T$, while $1$ in both $\calL'$ and $\calL'^T$, and there are at most $O(1)$ many of such edges by the bounded-degree assumption.   
% \end{enumerate}
% Combining the above, we have a change of \[ 
% \frac{\vtxcost(\calL')}{\vtxcost(\calL)}= \Delta(v) \cdot \Delta(u) \cdot \Delta( \edgeval(u,v)) \geq \frac{1}{q^{O(1)}}\cdot \sqrt{\wt(v)}\cdot \frac{1}{q^{O(1)}}\gg 1
% \]
% where we use our assumption $q = O(\wt(v)^\delta)$. Applying this argument inductively on the $H$ edge in the order of the distance from $U_\al$ completes our proof.
% \end{proof}
\begin{comment}
\subsection{Building the separator and bounding block-value by separators}
For each block through the walk, fixing the traversal direction from $U_\al$ to $V_\al$, consider the following set $S$,\begin{enumerate}
    \item We include a vertex into the separator $S$ if it is making its middle appearance; 
    \item We include a vertex from $U_\al$ into the separator if it is not making its \emph{last} appearance;
    \item We include a vertex from $V_\al$ into the separator if it is not making its \emph{first} appearance;
    \item We include any vertex from $U_\al\cap V_\al$ into the separator.
\end{enumerate}

\begin{claim}\label{claim:separator}
$S$ is a separator for each block.
\end{claim}
\begin{proof}
Take a path that is not blocked by $S$, its vertex in $U_\al$ must be making its last appearance, while the vertex in $V_\al$ is making its first appearance. Moreover, since any vertex between is either making the first or the last appearance, we can see that there must be some edge between a vertex with one endpoint making the first appearance and the other endpoint the last appearance, i.e., this edge is new  and does not appear in future block. This violates the evenness of our walk.
\end{proof}

\begin{definition}[Left/right separator boundary $S_L, S_R$]
For a given separator, we define the left (right) separator $S_L$ ( $S_R$) to be the set of vertices in $S$ reachable from $U_\al$ ( $V_\al$) without passing through any other vertex in $S$.
\end{definition}


% \paragraph{From separator to structure lemmas}
% \begin{lemma}
% Let $S$ be a given separator, and let $\calL$ be an edge-labeling that labels each edge $\{F,R,S,H\}$ consistent to the given separator, there is an \emph{optimal} labeling $\calL(S)$ that does not use any $S$ edge such that \[ 
% \sum_{\calL:\text{edge-labeling for } S} B_S(\calL) \leq \left(1+o_d(1)\right) B_S(\calL(S))
% \] 
% \end{lemma}


\paragraph{Accounting block value}
For each block $\al$, we start by fixing the traversal direction from $U$ to $V$, the vertex factors are accounted as the following,\begin{enumerate}
    \item For starters, we will presume any $R$ edge to have their destination fixed modulo the cost of $\pur$ throughout the walk, and notice that naively for each block $\al_i$, we would require $\pur(\al_i)$ factor to settle any confusion in this block, it suffices for us to assign the factors such that we charge the $\pur$ factor's receiver to the giver, i.e., let $\pur(\al_i)$ be the $\pur$ factor incurred by the walk on block $\al_i$;
    \item For vertices reachable from $U_\al$ without passing through $S$ (including those on the boundary), they are either already identified from the previous block in $U_\al$, or reached using an $R$ edge, hence no vertex cost is needed;
    \item For vertices reachable from $V_\al$ without passing through $S$ (and which are not in $S$ themselves), they are making their first appearance and hence a cost of $[d]$ (or $[m]$) is sufficient;
    \item Floating components: for components not reachable from $S$ that is also not reachable from $U_\al \cup V_\al$, all its vertices are making the first or last appearances, in which case, a label in $[n]$ per vertex for each new vertex, and a label in $2|V(\al)|q$ is sufficient for one vertex, and any other vertex can be reached using an $R$ edge for free.
    \item Each vertex on the the boundary of the separator $S_L$ is reached using an $R$ edge, hence no vertex factor; each vertex in the interior of the separator $S\setminus S_L$ is reached using an $H$ or $S$ edge, hence a cost of at most $q^{O(1)}$ per edge is sufficient (assuming each $H$ and $S$ edge gets assigned $O(1)$ $\pur$ factors);
    \item Each components of the separator $S$ not reachable from $S_L\cup S_R$ contributes a label in $2|V(\al)|q$.
\end{enumerate}

On the other hand, if we traverse from $V$ to $U$ for the same block,
\begin{enumerate}
    \item For vertices reachable from $V_\al$ without passing through $S$, they are either already identified from the previous block in $V_\al$, or reached using an $R$ edge, hence no vertex cost is needed;
    \item For vertices reachable from $U_\al$ without passing through $S$  (and which are not in $S$ themselves), they are making their first appearance and hence a cost of $[d]$ (or $[m]$) is sufficient;
    \item For components not reachable from $S$ that is also not reachable from $U_\al \cup V_\al$, all its vertices are making the first or last appearances, in which case, a label in $[n]$ per vertex for each new vertex, and a label in $2|V(\al)|q$ is sufficient for one vertex, and any other vertex can be reached using an $R$ edge for free. 
    \item Each vertex on the the boundary of the separator $S_R$ is reached using an $R$ edge, and any vertex in the interior of the separator $S\setminus S_L$ is reached using an $H$ or $S$ edge, hence a cost of at most $q^{O(1)}$ per edge is sufficient (assuming each $H$ and $S$ edge gets assigned $O(1)$ $\pur$ factors);
    \item Each components of the separator $S$ not reachable from $S_L\cup S_R$ contributes a label in $2|V(\al)|q$.
\end{enumerate}

We are now ready to summarize the block value.
\begin{enumerate}
    \item Each vertex outside the separator $S$ contributes a factor of its weight (either $d$ or $m$ depending on its vertex-type) in exactly one traversal direction, hence the factor of $\sqrt{\wt(i)}$ for each vertex $i\in V(\al)\setminus S$;
    \item Each vertex outside the separator that contributes a factor of its weight in both direction must be outside $U_\al\cup V_\al$ and it makes appearance in exactly one block, that said, each incident edge must be of even multiplicity (including $0$), and any such vertex contributes an extra factor of $\sqrt{\wt(i)}$ (and call any such vertex isolated);
    \item Each floating component not connected to $S$ receives an extra floating overhead for the $R$ return that is $2|V(\al)|q$ in one direction; and floating component connected to $S$ receives a label in $2|V(\al)|q$ in both directions, and it suffices for us to assign a $2|V(\al)|q$ factor for both direction regardless of connectivity to $S$;
    \item Each edge outside the separator is an $F/R$ edge, and gets assigned a factor of $\edgeval(F,R)$ depending on the edge-type, and each edge inside the separator is either $S$ or $H$ edge, and it suffices for us to assign a factor of $\edgeval(H)$ provided $\edgeval(H)\geq \edgeval(F,R)$. 
\end{enumerate}
This gives us a bound for $\al$ block for a given separator $S$,  \begin{align*}
B(\al) &\leq \pur(\al) \cdot \prod_{i\in V(\al)\setminus S}\sqrt{\wt(i)}^{1+1_{iso}(i)} \prod_{e\in E(S)} q^{O(1)} \cdot (2|V(\al)|q)^{2|\float(\al)|} \\&\cdot \prod_{e \in E(\al)\setminus E(S)}\edgeval(F,R) \cdot \prod_{e\in E(S)} \edgeval(H)    
\end{align*}


where $\pur(\al)$ is the potential-unforced-return factor incurred by the walk of this current block.
\end{comment}
\subsection{Applying block function to our matrices}
We now combine the above block-function with our $\pur$ bounds.
\subsubsection{Block function for $A^{-1}$-terms}

\begin{lemma}[Block-value bound for $A^{-1}$] For any shape $\al$ that appears in decomposition of $A^{-1}$, we have the following block-value bound,
\[ 
B(\al) \leq  \sum_{S:\text{separator}} \prod_{i\in V(\al)\setminus S}\sqrt{\wt(i)} \prod_{e\in E(S)} q^{O(1)} \cdot \prod_{e \in E(\al)\setminus E(S)}\edgeval(F,R) \cdot \prod_{e\in E(S)} \edgeval(H)
\]
\end{lemma}

\begin{proof}
Recall that our bound $\pur$ bounds for $A^{-1}$ states that \[ 
\pur_t(v)\leq 4s_t(v) + 4h_t(v)
\]
That said, for each vertex in the block, we do not incur any change in the $\pur$ factor unless there is a surprise visit or $H$-visit going into the vertex. Via our separator construction, any $S/H$ edge is inside the separator and therefore, we can bound the change of $\pur$ factors charged to the current block by\[ 
\sum_{v\in V(\al_i)}\left( \pur_{i}(v) - \pur_{i-1}(v)\right)  \leq O(1) |E(S)|
\]
Finally since each $\pur$-confusion can be settled via a label in $4q$, and there is no floating component for terms in $A^{-1}$, the bound follows after summing over all possible separators.
\end{proof}

\subsubsection{Block function for non-intersecting $\tau(R)$-terms}
\begin{definition}[Canonical $\tau(R)$-ordering for traversal]
For a given shape from $\tau(R)$, we consider a fixed order of traversing edges for encoding:
\begin{enumerate}
    \item First traverse the $U-V$ path that passes through a square vertex, in particular, traverse both edges on the $U-V$ path from $U\cup V$;
    \item Starting from the first square vertex, traverse edges from each $A^{-1}$ gadget;
    \item Traverse the edges from the filling layer;
    \item Traverse the edges in the second $A^{-1}$ gadget if available;
    \item Traverse the $H_2$ attachment gadget.
\end{enumerate}
\end{definition}
\begin{remark}
Each vertex being traversed in the canonical ordering satisfies the following: \begin{enumerate}
    \item Any square vertices $u$  pushes out $2 + dormant(u) $ edges where $dormant(u)$ is the number of $M_D$ edges it pushes out to circle vertices;
    \item Any circle vertex pushes out $1$ edge.
\end{enumerate}
\end{remark}


We first apply the block-function for $\tau(R)$ terms, i.e., non-intersecting terms in $R$. Recall that we have the following bounds for $\pur$ in the $R$-terms, where it is important to distinguish between circle and square vertices, that is \[ 
\pur_t(v) \leq 2s_t(v) + h_t(v)
\]
for a circle vertex $v$, and \[ 
\pur(u) \leq (3+\text{dormant}(u)  \cdot \text{middle-appear}(u ) \leq O(1) \cdot \text{middle-appear}(u )
\]
for a square vertex $u$ where the second inequality follows from our truncation that each square vertex may push out at most $3\leq O(1)$ dormant edges each time it appears (as otherwise the gap from excess $H_2$ edges is sufficient for us to bypass a tight analysis via trace moment method).

For non-intersecting terms in $\tau(R)$, traversing each shape following the canonical ordering ensures that each circle vertex pushes out at most $1$ edge, hence our return bound from earlier applies.  Moreover, notice each square vertex, if contributing to $\pur$-factor via making a middle-appearance, is also included into the separator by definition. That said, each square vertex either contributes a factor of $\sqrt{m}$ (by being outside the separator), or $q^{O(1)}$ when making a middle appearance (while inside the separator) but not both at the same time, we have \begin{align*}
&B(\al) \leq  \sum_{S:\text{separator for }\al } 
\prod_{i\in V(\al)\setminus S}\sqrt{\wt(i)} \prod_{e\in E(S)} q^{O(1)}  \\&\cdot  \prod_{e \in E(\al)\setminus E(S)}\edgeval(F,R) \cdot \prod_{e\in E(S)} \edgeval(H) \prod_{\substack{i\in S\\ \text{square}}  } q^{O(1)} \cdot (2|V(\al)|q)^{2|\float(\al)|} 
\end{align*}

% \paragraph{From structure lemmas to separators}
% With the above structure lemmas for locally optimal edge-labeling, we are now ready to relate the block value to the separator. For starters, we observe that given a locally optimal edge-labeling $\calL_{U\rightarrow V}$ , we can define a set of vertices $S(\calL_{U\rightarrow V})$ such that \begin{enumerate}
%     \item We include any vertex incident to both $F$ and $R$ edge into $S$;
%     \item We include vertex in $U_\al$ into $S$ if it is only incident to $F$ edges, and connected to $V_\al$ ;
%     \item We include vertex in $V_\al$ into $S$ if it is only incident to $R$ edges, and connected to $V_\al$;
%     \item We include any vertex in $U_\al\cap V_\al$ into $S$.
% \end{enumerate}
% We observe that $S(\calL_{U\rightarrow V})$ is a separator since \begin{enumerate}
%     \item Any path from $U_\al$ to $V_\al$ is of the structure $R\rightarrow F$ though the edge-set may be empty;
%     \item Any path that witnesses a turn from $R$ to $F$ passes through a vertex included by (1);
%     \item Any other path is either all $F$ or all $R$ and passes through a vertex either in $U_\al$ or $V_\al$ by (2) or (3);
%     \item Any vertex in $U_\al\cap V_\al$ is in the mandatory separator and included by (4).
% \end{enumerate}
% \begin{proposition}[Separator is invariant of traversal-direction]
% Given an edge-labeling $\calL$ (presumed to be traversed from $U$ to $V$, \[ 
% S(\calL_{U\rightarrow V}) = S(\calL^T_{V\rightarrow U})
% \]
% Furthermore, we can simply write the separator as $S(\calL)$.
% \end{proposition}

% \begin{proposition}
% For a bounded degree shape, given an edge labeling $\calL$ and its corresponding separator $S$, we can bound its block value by \[ 
% B(\calL) \leq \prod_{i\in V(\al)\setminus S} \wt(i)^{\frac{1}{2}+\frac{1}{2} 1_{i \text{ is isolated} } }  
% \]
% \end{proposition}
% \begin{proof}

% \end{proof}

% \begin{corollary}
% For the particular shape defined above, assuming $m<\frac{d^2}{4}$, we obtain a bound of \[ 
% \|M_\al\|\leq 2\cdot \frac{1}{d^2} \sqrt{md^2}
% \]
% where we recall the factor $\frac{1}{d^2}$ comes from normalization.
% \end{corollary}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

% Common
\def \N {\mathbb{N}}
\def \R {\mathbb{R}}
\def \C {\mathbb{C}}
\def \Q {\mathbb{Q}}
\def \Z {\mathbb{Z}}
\def \F {\mathbb{F}}
\def \E {\mathbb{E}}
\def \PE {\wt{\mathbb{E}}}
\def \eps {\epsilon}
\def \al {\alpha}
\renewcommand{\Pr}{\mathop{\bf Pr\/}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ot}{\otimes}
\newcommand{\zo}{\{0,1\}}
\newcommand{\pmo}{\{\pm1\}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\imp}{\Longrightarrow}
\newcommand{\brac}[1]{\left\langle #1 \right\rangle}
\newcommand{\KL}{d_{\mathrm{KL}}}
\newcommand{\TV}{d_{\mathrm{TV}}}
\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
 \def\1{\bm{1}}
\def \st {\text{s.t.}}
\newcommand{\TODO}[1]{\textcolor{red}{#1}}
\newcommand{\calF}{\mathcal{F}}
% mathsf 
\newcommand{\SA}{\mathsf{SA}}
\newcommand{\SOS}{\mathsf{SOS}}

% complexity classes
\newcommand{\PTIME}{\mathsf{P}}
\newcommand{\LOGSPACE}{\mathsf{L}}
\newcommand{\ZPP}{\mathsf{ZPP}}
\newcommand{\RP}{\mathsf{RP}}
\newcommand{\BPP}{\mathsf{BPP}}
\newcommand{\NP}{\mathsf{NP}}
\newcommand{\coNP}{\mathsf{coNP}}
\newcommand{\MA}{\mathsf{MA}}
\newcommand{\PH}{\mathsf{PH}}
\newcommand{\TC}{\mathsf{TC}}
\newcommand{\AC}{\mathsf{AC}}
\newcommand{\SC}{\mathsf{SC}}
\newcommand{\SZK}{\mathsf{SZK}}
\newcommand{\AM}{\mathsf{AM}}
\newcommand{\IP}{\mathsf{IP}}
\newcommand{\PSPACE}{\mathsf{PSPACE}}
\newcommand{\EXP}{\mathsf{EXP}}
\newcommand{\MIP}{\mathsf{MIP}}
\newcommand{\NEXP}{\mathsf{NEXP}}
\newcommand{\BQP}{\mathsf{BQP}}
\newcommand{\PP}{\mathsf{PP}}
\newcommand{\SP}{\mathsf{\#P}}

% Environments
% \renewenvironment{proof}{{\emph{Proof.}  }}{\hfill$\square$ \vspace{8pt}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{question}[theorem]{Question}
\newtheorem{answer}[theorem]{Answer}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem{exercise}[theorem]{Exercise}
% \theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Example}

% Math terms
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\size}{\textnormal{size}}
\newcommand{\avg}{\mathop{\textnormal{avg}}}
\newcommand{\sgn}{\textnormal{sgn}}
\newcommand{\dist}{\textnormal{dist}}
\newcommand{\vol}{\textnormal{vol}}
\newcommand{\spn}{\textnormal{span}}
\newcommand{\supp}{\textnormal{supp}}
% \newcommand{\tr}{\operatorname{tr}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\conv}{\operatorname{conv}}


% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\valpha{{\bm{\alpha}}}
\def\vbeta{{\bm{\beta}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathcal{A}}}
\def\sB{{\mathcal{B}}}
\def\sC{{\mathcal{C}}}
\def\sD{{\mathcal{D}}}
\def\sE{{\mathcal{E}}}
\def\sF{{\mathcal{F}}}
\def\sG{{\mathcal{G}}}
\def\sH{{\mathcal{H}}}
\def\sI{{\mathcal{I}}}
\def\sJ{{\mathcal{J}}}
\def\sK{{\mathcal{K}}}
\def\sL{{\mathcal{L}}}
\def\sM{{\mathcal{M}}}
\def\sN{{\mathcal{N}}}
\def\sO{{\mathcal{O}}}
\def\sP{{\mathcal{P}}}
\def\sQ{{\mathcal{Q}}}
\def\sR{{\mathcal{R}}}
\def\sS{{\mathcal{S}}}
\def\sT{{\mathcal{T}}}
\def\sU{{\mathcal{U}}}
\def\sV{{\mathcal{V}}}
\def\sW{{\mathcal{W}}}
\def\sX{{\mathcal{X}}}
\def\sY{{\mathcal{Y}}}
\def\sZ{{\mathcal{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\Ls}{\mathcal{L}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\cl}{\text{cl}}
% \newcommand{\1}[1]{\mathds{1}\left[#1\right]}


% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\seq}{\subseteq}

\renewcommand{\wt}{\mathsf{weight}}

\mathchardef\mhyphen="2D
\newcommand{\val}{\text{val}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calI}{\mathcal{I}}

% shape terms
\newcommand{\midshape}{\mathsf{MidShape}}
\newcommand{\leftshape}{\mathsf{LeftShape}}
\newcommand{\rightshape}{\mathsf{RightShape}}
\newcommand{\dsos}{\mathsf{dsos}}
\newcommand{\mul}{\text{mul}}
\newcommand{\ind}[1]{1_{{#1}}}
\newcommand{\din}{d_{\text{in}}}
\newcommand{\dout}{d_{\text{out}}}
\newcommand{\sbm}{D_{\text{SBM}}}
\newcommand{\cycle}{\ind{\calE}}
\newcommand{\bdd}{\ind{\calF}}
\newcommand{\exc}{\mathsf{excess}}
\newcommand{\cc}{\mathsf{\#cc}}
%\newcommand{\vtxcoef}{\mathsf{vtxcoef}}
\newcommand{\float}{\mathsf{float}}
\newcommand{\fs}{\mathsf{float \mhyphen stick}}
\newcommand{\fc}{\mathsf{float\mhyphen cyc}}
\newcommand{\cyclen}{\mathsf{cyclen}}
\newcommand{\mvs}{\text{MVS}}
\newcommand{\smvs}{\text{SMVS}}
\newcommand{\dang}{\mathsf{dangling}}
\newcommand{\gam}{\gamma}
\newcommand{\Id}{\text{Id}}
\newcommand{\trivial}{\text{trivial}}
\newcommand{\cval}[1]{\mathsf{Colorval}[#1]}	
\newcommand{\crosscol}{\text{cross-color}}
\renewcommand{\int }{\text{Int}}
\newcommand{\slack}{\text{slack}}
\newcommand{\Glyph}{\mathcal{G}}
\newcommand{\glyph}{\tex{glyph}}
\newcommand{\yes}{\text{Yes}}
\newcommand{\no}{\text{No}}
\newcommand{\mix}{\text{Mix}}
\renewcommand{\cp}{\text{CP}}
\newcommand{\pure}{\text{pure-color}}
\newcommand{\depth}{\text{depth}}
\newcommand{\res}{\text{res}}
\newcommand{\girth}{\text{girth}}
\newcommand{\vap}{\text{vap}}
\newcommand{\boundary}{\text{boundary}}
\newcommand{\chunk}{\text{chunk}}
\newcommand{\cm}{M^{(c)}}
\renewcommand{\phantom}{\text{phantom}}
\newcommand{\exwedge}{\text{exc-wedge}}
\newcommand{\cnorm}{c_{\mathsf{norm}}}
\newcommand{\ceta}{c_\eta}
\newcommand{\edgeco}{\left(\eta\cdot\sqrt{\frac{d}{n}} \right)}
\newcommand{\vtxco}{\left(\frac{1}{k}  \right)}
\newcommand{\sval}{\text{SMVS-val}}
\newcommand{\fantome}{\text{distinct phantom}}
\newcommand{\iso}{\mathsf{\# isolated}}
\newcommand{\isocc}{\mathsf{\#isocc}}
\newcommand{\cnt}{\mathsf{count}}
\newcommand{\gp}{{\gamma'}}
\renewcommand{\cp}{\text{CP}}
\newcommand{\col}{\text{color}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\aut}{\mathsf{Aut}}
\newcommand{\nontrivial}{\mathsf{non-trivial}}
\newcommand{\vtxcost}{\mathsf{vtxcost}}
\newcommand{\edgeval}{\mathsf{edgeval}}
%\newcommand{\cs}{\mathsf{Color-shape}}
\DeclareMathOperator{\pE}{\widetilde{\E}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}




==> prelims.tex <==
\section{Preliminaries}

The \emph{univariate Hermite polynomials} $\{h_k\}_{k\in \N}$ are defined by the following recurrence:
\begin{equation*}
    h_0(x) = 1, \quad h_1(x) = x, \quad h_{k+1}(x) = xh_k(x) - k h_{k-1}(x) \mper
\end{equation*}
We further define the normalized Hermite polynomials $\wt{h}_k(x) = \frac{1}{\sqrt{k!}} h_k(x)$.

We will need the following facts about Hermite polynomials:
\begin{fact} \label{fact:hermite-even-odd}
    For even $k$, $h_k(x) = h_k(-x)$ for all $x\in\R$.
    For odd $k$, $h_k(x) = -h_k(-x)$ for all $x\in\R$.
\end{fact}


==> psdmass.tex <==
\section{Analysis for $\Lambda_\trivial$}

We first recall that \[ 
\Lambda_\trivial = \sum_{i\in [m]} w_\trivial[i] v_iv_i^T
\]
for \[ 
w_\trivial = M^{(-1)}_\trivial \cdot 1_m = \left(I-\frac{c_s}{d}\cdot J_m \right) 1_m  = (1- \frac{c_s \cdot m}{d}) 1_m
\]
Therefore, we have \[ 
\Lambda_\trivial = (1-\frac{c_s\cdot m}{d})\sum_{i\in [m]} v_iv_i^T
\]
\begin{claim}
We can pick $m = \frac{d^2}{4\cdot c_\eta}$ for some $c_\eta>1$  such that for any $c>0$, we have \[ 
\frac{c_s \cdot m }{d} <c
 \]
\end{claim}
\begin{proof}
Recall that \[ 
c_s = \frac{1}{1 + \frac{1}{d} 1^T_m A^{(-1)} 1_m}
\]
and \[ 
\lambda_{\min}(A^{(-1)}) \geq 1 - \|M_\tau\| > 1 - 2\sqrt{md^2}\cdot \frac{1}{d^2} = 1- \frac{1}{\sqrt{c_\eta}}
\]
Therefore, \[
c_s < \frac{1}{1+ \frac{1}{d} m (1- \frac{1}{\sqrt{c_\eta}}) }\approx \frac{1}{1-\frac{1}{\sqrt{c_\eta}}} \frac{d}{m}
 \]
 Thus we need to have
\end{proof}

==> truncation.tex <==
\section{Large shapes are negligible}
To add truncation terms as we. are just applying matrix norm bounds to shapes that are not too large. For the large ones, frobenius norm should be enough.
